A Large-Scale Comparison of Tetrahedral and Hexahedral Elements for Solving Elliptic PDEs with the Finite Element Method

The Finite Element Method (FEM) is widely used to solve discrete Partial Differential Equations (PDEs) in engineering and graphics applications. The popularity of FEM led to the development of a large family of variants, most of which require a tetrahedral or hexahedral mesh to construct the basis. While the theoretical properties of FEM basis (such as convergence rate, stability, etc.) are well understood under specific assumptions on the mesh quality, their practical performance, influenced both by the choice of the basis construction and quality of mesh generation, have not been systematically documented for large collections of automatically meshed 3D geometries. We introduce a set of benchmark problems involving most commonly solved elliptic PDEs, starting from simple cases with an analytical solution, moving to commonly used test problem setups, and using manufactured solutions for thousands of real-world, automatically meshed geometries. For all these cases, we use state-of-the-art meshing tools to create both tetrahedral and hexahedral meshes, and compare the performance of different element types for common elliptic PDEs. The goal of his benchmark is to enable comparison of complete FEM pipelines, from mesh generation to algebraic solver, and exploration of relative impact of different factors on the overall system performance.

==> 98-cover-letter.tex <==
Dear Editor,

We submit our manuscript entitled ``A Large-Scale Comparison of Tetrahedral and Hexahedral Elements for Finite Element Analysis'' to your consideration for publication in the ACM Transaction on Graphics.

We believe that the work, which contains the first large scale evaluation of discretizations on thousand of real-world models for Finite Element Analysis, will be of high interests to the readers of the journal. It provides new insights that we believe will provide a guide in the development of new meshing and FEA techniques and a standard set of benchmark problems to quantitatively evaluate new techniques.

We commit on publicly releasing the experimental description, meshes, and reference implementation of our testing infrastructure in the additional material.

Sincerely,
The Authors

